Modeling of Chemical Reactions in Rarefied Gas Flows by the Kinetic Fokker-Planck Method

We propose a novel approach for modeling chemical reactions within the particle-based Fokker-Planck framework for gas flow simulations which conserves mass, momentum, and energy while retaining the performance advantages of the Fokker-Planck approach over the Direct Simulation Monte Carlo (DSMC) method in areas of high density. We show an application of the approach to recombination and exchange reactions, discuss verification results, and demonstrate performance advantages when compared to DSMC for applications in low Knudsen number regimes. The developed method can be applied to simulation of flows in the continuum and transitional regimes, as well as to multi-scale coupled Fokker-Planck-DSMC simulations.

==> content/air_chemistry.tex <==
\section{Modeling of Air Chemistry}
In this section, we present results for a coupled air chemistry simulation using 15 dissociation reactions from Tables \ref{tab:air_chemistry_o2_diss}, \ref{tab:air_chemistry_n2_diss}, and \ref{tab:air_chemistry_no_diss}, along with the 2 exchange reactions listed in Table~\ref{tab:air_chemistry_exchange}.
The simulation setup was chosen to be the same as described in Section \ref{sec:reaction_kinetcs_k_T}.
For this analysis, only the continuum model and the FP results were considered, as they share the closest modeling assumptions.

As in previous results, the development of translational temperature agrees very well between the two models, as shown in Fig.~\ref{fig:temp_air}.
%----------------------------------------------------------------------------------------------------------------------
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/air_chemistry/temp_air_new.png}
    \caption{\label{fig:temp_air} Temperature using air reactions.}
\end{figure}
%----------------------------------------------------------------------------------------------------------------------
Also the development of the number densities, seen in Fig.~\ref{fig:nrho_air} shows a good agreement even in the very numerically stiff section at the beginning of the simulation.
%----------------------------------------------------------------------------------------------------------------------
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/air_chemistry/nrho_air_new.png}
    \caption{\label{fig:nrho_air} Number density using air reactions.}
\end{figure}
%----------------------------------------------------------------------------------------------------------------------
However, the differences increase as the simulation progresses.
These differences can be better understood when only looking at the reaction kinetics of \ch{NO}, \ch{N2}, and \ch{N} as seen in Figure~\ref{fig:nrho_air_NO_N2_N}.
While the reaction kinetics of \ch{NO} and \ch{N} show a very similar qualitative behavior between the models, there is clearly a difference in the decay of \ch{N2}.
%----------------------------------------------------------------------------------------------------------------------
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/air_chemistry/nrho_air_NO_N2_N.png}
    \caption{\label{fig:nrho_air_NO_N2_N} Number density of \ch{NO}, \ch{N2}, and \ch{N} using air reactions.}
\end{figure}
%----------------------------------------------------------------------------------------------------------------------
Some of the reactions involving NO proceed on very short time-scales, and the results are strongly affected by the choice of timestep and time-stepping scheme, as this rapid evolution of the system at the start of the simulation needs to be resolved.
In addition, even small differences in temperature can skew the the kinetics.
Those differences in the translational temperature can be explained by differences in the relaxation of vibrational energies as seen in Fig.~\ref{fig:tvib_air}, which, as discussed
above, is attributed to the differences between the vibrational relaxation modelling between the continuum- and particle-based approaches.
%----------------------------------------------------------------------------------------------------------------------
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/air_chemistry/tvib_air.png}
    \caption{\label{fig:tvib_air} Temperature using air reactions.}
\end{figure}

Nonetheless our model is able to achieve a good agreement with the continuum model even for this large and stiff system.
The observed maximum relative differences between the different methods for the number densities of all species apart from \ch{O2} do not exceed 10 - 13\%. For \ch{O2} the difference is larger (up to 100\%) due to its number density approaching zero as the simulation processes. Therefore, even minor difference in reaction rates lead to large relative changes in the number density; however, the absolute values remain negligibly small.
The maximum relative difference for the temperature is around 2\%.


==> content/introduction_old.tex <==
\section{Introduction}
Flows encountered in space applications, like atmospheric reentry or thruster plume expansion and interactions, can be described by the well-known Boltzmann equation.
A common approach to solve it numerically is the Direct Simulation Monte-Carlo (DSMC) method pioneered by Bird \cite{bird_molecular_1994}.
The method is very efficient for high Knudsen numbers but becomes increasingly computationally intensive when approaching the continuum limit.
In this regime the Boltzmann equation can be numerically solved using the kinetic Fokker-Planck (FP) method \cite{jenny_solution_2010} which, like DSMC, relies on simulated particles to model the transport of mass, momentum and energy through the flow domain, but unlike DSMC does not resolve individual collisions.
Due to the similarity in their formulation a hybrid method based on DSMC and FP can also be derived which allows for a computationally efficient simulation of flows with a broad range of Knudsen numbers \cite{gorji_fokkerplanckdsmc_2015}.
In the last years, the FP model has been extended to describe diatomic \cite{gorji_fokkerplanck_2013,hepp_master_2020} and polyatomic \cite{mathiaud_fokkerplanck_2017, aaron_nagel_modeling_2023} [\hl{my RGD paper}] gases for single species  as well as for mixtures \cite{hepp_kinetic_2020,hepp_kinetic_2020-2}.

\hl{Below is a part discussing modelling of chemistry in non-equilibrium flows in general. Need to somehow make it fit better with the other parts in the introduction. Perhaps put the FP stuff afterwards, saying that basically a lot of the methods (Chapman-Enskog, DSMC, etc.) have considered chemical reactions, but in FP it's basically an open topic without prior work.}
In rarefied regimes, the distributions of the particles' velocities and internal energies can deviate from the equilibrium Maxwell-Boltzmann statistics, which in turn can affect reaction rates, and needs to be accounted for in flow simulations. First theoretical works in the field considered the impact of non-equilibrium velocity distributions on chemical reaction rates~\cite{prigogine1949perturbation,takayanagi1951theory,shizgal1970nonequilibrium} via the Chapman--Enskog method; this impact was also observed in DSMC simulations~\cite{lemarchand1998perturbation}. More recent results for reacting flows with non-equilibrium velocity distributions include the proof of the existence of a stable equilibrium solution of the Boltzmann equation for reacting flows~\cite{rossani1999note}, and development of moment-based approaches~\cite{sarna2021moment}. The approach based on the Chapman--Enskog expansion has been also extended to polyatomic gas flows in thermal equilibrium~\cite{kustova2011cross} and non-equilibrium~\cite{kolesnichenko2010gas,kustova2015reaction}.

In the Direct Simulation Monte Carlo method, the most widely used approach to simulation of chemical reactions remains the Total Collision Energy (TCE) model~\cite{bird_molecular_1994,bird_chemical_2011}, which aims to reproduce the Arrhenius law in the equilibrium case. However, the model is not necessarily valid outside of equilibrium; it also places restrictions on the constant appearing in the Arrhenius law (thus, not every Arrhenius curve fit can be represented in TCE) and the internal energies (which are assumed to be continuous). Various modifications to the model have been proposed~\cite{wadsworth1997vibrational,gimelshein_use_2004} to address these issues, however, the standard formulation remains perhaps the most widely-used one due to its simplicity. Recent simulations coupling DSMC and molecular dynamics simulations (with the coupled approach referred to by the authors as ``Direct molecular simulation'') have confirmed the role of coupling between internal energy relaxation and chemical reactions~\cite{grover2019direct}, thus again highlighting the need for chemical reaction models that account for non-equilibrium effects.

Finally, approaches to simulation of chemically reacting flows based on the model Bhatnagar--Gross-Krook (BGK) equations should be mentioned~\cite{groppi2004bhatnagar,monaco2005bgk,baranger2020bgk}. These approaches have so far been applied only to continuum flows; moreover, due to the use of the BGK approximation, they assume an equilibrium velocity distribution.

\hl{Since the goal of the Fokker--Planck is to efficiently simulate gas flows in the continuum limit, the role of the aforementioned non-equilibrium effects is expected to be less significant.}

%Chemistry - here I need more litrature
However, the modeling of chemical reactions via the kinetic FP method remains an open research topic.
Many problems arise from the fact that properties of the reactants need to be considered to evaluate a chemical reaction.
This contradicts the FP approach that achieves its linear scaling in terms of particle numbers by forgoing the evaluation of interaction pairs.
In this paper we propose a novel approach to model chemical reactions via our cubic FP method implemented in the SPARTA framework \cite{plimpton_direct_2019}.
The model conserves mass, energy and momentum while retaining the performance advantages in areas of low Kn numbers. It is verified by comparison to continuum-based analytical and numerical solutions.

The paper is structured as follows: first, an overview of the Fokker-Planck method is given. Its extension to chemically reacting flows is then proposed. Comparisons to analytical and numerical solutions are then presented for various testcases. Finally, an analysis of the computational performance of the model in comparison to DSMC is provided.

==> content/old_energy_conservation.tex <==
\subsubsection{OLD Energy conservation}
Given as set of reactions that took place $R$ we want the energy of the reactants be equal to the energy of the products such
\begin{equation}
	\sum_j^R e_{\mm{reac}, j} \overset{!}{=} \sum_j^R e_{\mm{prod}, j}.
\end{equation}
For the reactants we assume that the energy of all participants in the reaction $j$ can be expressed as the sum of the kinetic and internal energies
\begin{equation}
	e_{\mm{reac}, j}  = \sum_r \big( e_{\mm{kin}, j, r} + e_{\mm{int}, j, r} \big).
\end{equation}
For the energy of the products we state that the energy is the sum of the centre of mass energy $e_{\mm{cm}}$, the collision energy $e_{\mm{coll}}$, and the energy of the reaction $\Delta e$ which is negative or positive depending whether or not the reaction is exo- or endothermic.
\begin{equation}
	e_{\mm{prod}, j} = e_{\mm{cm}, j} + e_{\mm{coll}, j} + \Delta e_j.
\end{equation}
The collision energy in this case is the sum of the relative kinetic energy of the particles plus the internal energy of all participating internal degrees of freedom \cite{bird_molecular_1994}.
The total energy equation can thus be stated as
\begin{equation}
	\label{eqn:e_react}
	\sum_j^R \sum_r \big( e_{\mm{kin}, j, r} + e_{\mm{int}, j, r} \big) \overset{!}{=} \sum_j^R \big( e_{\mm{cm}, j} + e_{\mm{coll}, j} + \Delta e_j \big).
\end{equation}
Since we are only interested in conserving the total energy of all reactions that took place we can rewrite Eqn.~(\ref{eqn:e_react}) using the total energy as
\begin{equation}
	E_{\mm{kin}} + E_{\mm{int}} \overset{!}{=} E_{\mm{cm}} + E_{\mm{coll}} + \Delta E.
\end{equation}
The left hand side of the equation above is given by the particles selected for the reactions.
On the right hand side the centre of mass energy $E_{\mm{cm}}$ is set due to momentum conservation and the total $\Delta E$ is given by the physics of the reactions.
To fulfill the equation we now need to adjust the "assumed" collision energy of the products (the assumption was based on averages) to  the real energy of the selected particles in the form.
Now we can scale $e_{\mm{coll}, j}$ of each reaction $j$ to fulfill the energy conservation in the cell as
\begin{equation}
	\frac{e'_{\mm{coll}, j}}{e_{\mm{coll}, j}} = \frac{E_{\mm{kin}} + E_{\mm{int}} - (E_{\mm{cm}} + \Delta E)}{E_{\mm{coll}}}.
\end{equation} 
For the equation to be realizable the following inequality must be fulfilled:
\begin{equation}
    E_{\mm{kin}} + E_{\mm{int}} \geq E_{\mm{cm}} + \Delta E.
\end{equation}
This inequality can be written in a stronger form as
\begin{align}
    \label{eqn:energy_conserv_kin_cm}E_{\mm{kin}} &\geq E_{\mm{cm}}\\
    \label{eqn:energy_conserv_int_delta}E_{\mm{int}} &\geq \Delta E.
\end{align}

We start by focusing on Eq.~(\ref{eqn:energy_conserv_kin_cm}).
The total kinetic energy $E_{\mm{kin}}$ of the reactants can be written as
\begin{equation}
	E_{\mm{kin}}  = \frac{1}{2} \sum_r^{N_r} m_r |\vec{v}_r|^2.
\end{equation}
Since we already set the centre of mass velocity of all products to conserve momentum we can write for the centre of mass energy $E_{\mm{cm}}$
\begin{equation}
	E_{\mm{cm}} = \frac{1}{2} |\vec{v}_{\mm{cm}}|^2 \sum_p^{N_p} m_p.
\end{equation}
Due to mass conservation we have
\begin{equation}
	\sum_p^{N_p} m_p = \sum_r^{N_r} m_r = M_r.
\end{equation}
With the definition for $v_{\mm{cm}}$
\begin{equation}
	\vec{v}_{\mm{cm}} = \frac{\sum_r^{N_r} m_r \vec{v}_r}{M_r}
\end{equation}
we can write $E_{\mm{cm}}$ as
\begin{equation}
	E_{\mm{cm}} = \frac{1}{2} M_r \left| \sum_r^{N_r} \frac{m_r}{M_r} \vec{v}_r \right|^2.
\end{equation}
Using the formulation for the kinetic and centre of mass energy in Eq.~(\ref{eqn:energy_conserv_kin_cm}) we get
\begin{equation}
	M_r \left| \sum_r^{N_r} \frac{m_r}{M_r} \vec{v}_r \right|^2 \overset{!}{\leq} \sum_r^{N_r} m_r |\vec{v}_r|^2.
\end{equation}
Since $M_r > 0$ we can write
\begin{equation}
	\left| \sum_r^{N_r} \frac{m_r}{M_r} \vec{v}_r \right|^2 \overset{!}{\leq} \sum_r^{N_r} \frac{m_r}{M_r} |\vec{v}_r|^2
\end{equation}
which is the Cauchy - Schwarz inequality and thus Eq.~(\ref{eqn:energy_conserv_kin_cm}) is always fulfilled.

Now focusing on Eq.~(\ref{eqn:energy_conserv_int_delta}) we can enforced the criterium by only selecting reactants to perform reaction $j$ for which it holds
\begin{equation}
	\sum_r e_{\mm{int}, r, j} \leq \Delta e_j.
\end{equation}
Since only the information about the kinetic particle is available at any point in time directly, we fulfill the equation by only allowing kinetic particles to partake in the reaction if
\begin{equation}
	e_{\mm{int}, \mm{kin}, j} + \sum_r \min\left(e_{\mm{int}}(s_r) \right) \leq \Delta e_j
\end{equation}
where $\min(e_{\mm{int}}(s_r))$ is the minimum internal energy of a particle in the current cell which belongs to the species $s$ of the reactant $r$.
This makes sure that Eq.~(\ref{eqn:energy_conserv_int_delta}) is always fulfilled thus leading to energy conservation.

==> content/pseudocode.tex <==
\section{Pseudo Code}
Here I want a pseudo code listing showing how the model works
\begin{figure}[ht]
	\centering
\begin{algorithm}[H]
	\SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{InOut}{InOut}
	\SetAlgoLined
	\InOut{list of cells $C$}
    \For{$\mm{each}$ $\mm{cell}$ c $\mm{in}$ C}{
        $P \gets$ list of particles in cell $c$\;
	    \For{$\mm{each}$ $\mm{particle}$ p $\mm{in}$ P}{
            check if $p.s$ was choses for reaction\;
        }
	}
	\caption{\label{alg:chemistry}Chemistry Model - General Overview}
\end{algorithm}
\end{figure}

==> content/verification.tex <==
\section{Verification}
In this section we provide verification results for our chemistry model based on comparisons to analytical solutions as well as 0D  simulation results created using multi-temperature continuum models as well as the SPARTA DSMC code \cite{plimpton_direct_2019}.
For the verification process, unless otherwise specified, we use Arrhenius-type rate constants $k$ of the form:
\begin{equation}
	\label{eqn:arrhenius}
	k(T) = A T^B \exp\left(-\frac{E_a}{\kb T} \right)
\end{equation}
where $A$ and $B$ are the Arrhenius coefficients, $T$ is the kinetic temperature, and $E_a$ is the activation energy.
Our proposed chemistry model is agnostic to the choice of rate constant. This means that other formulations of rate constants, such as Bird's Quantum-Kinetic model (QK) \cite{bird_q-k_2011} or tabulated values, can be used. Since the FP model is valid near the continuum regime, we use the Arrhenius equation for consistent comparisons with established Navier-Stokes models.

\subsection{Calculation of Rate Constants}
\label{sec:calculation_of_rate_constants}
As the first step of the verification process, we demonstrate that our model correctly reproduces the provided rate constants. To achieve this, a 0D FP simulation is run multiple times for selected temperature points using different random seeds. The number of evaluated reactions is then averaged over all executions and used to calculate the "effective" rate constant produced by our simulation. This rate constant is subsequently compared to the rate constant predicted by the Arrhenius model, as shown in Eqn.~(\ref{eqn:arrhenius}).

The chemical process in this case is a system of two coupled dissociation reactions
\begin{align}
    \ch{O2 + O2}&\overset{\textit{r} 1}{\longrightarrow}\ch{O2} + 2\ch{O}\\
    \ch{O + O2}&\overset{\textit{r} 2}{\longrightarrow}3\ch{O}
% 	\ch{O2 + O2 &->[\textit{r} 1] O2 + 2 O}\\
% 	\ch{O + O2 &->[\textit{r} 2] 3 O}
\end{align}
with the reaction rates being
\begin{align}
	r_1 &= k_1(T)[\ch{O_2}][\ch{O_2}]\\
	r_2 &= k_2(T)[\ch{O}][\ch{O_2}].
\end{align}
The simulation domain is a cube with a volume of $V = \SI{e-12}{\cubic\meter}$. 
We used a time step of $\Delta t = \SI{e-10}{\second}$, and a particle weight of $w=\num{e5}$.
The number densities at the beginning of the simulation where $n_{\ch{O}}(t_0) = \SI{e21}{\per\meter\cubed}$ and $n_{\ch{O2}}(t_0) = \SI{9.9e22}{\per\meter\cubed}$.
The used Arrhenius parameters can be found in Tab.~\ref{tab:air_chemistry_o2_diss}.
%\begin{table}[h!]
%\caption{\label{tab:reaction_rates_setup}Arrhenius Parameters for Coupled \ch{O2 + O} Dissociation}
%\centering
 %\begin{tabular}{l|ccc} 
%Reaction &  $A$ / $\left(\si{\meter\cubed\per\second\kelvin\tothe{-B}}\right)$  & $B$ & $E_a$ / $\si{\joule}$\\
 %\hline
%\ch{O2 + O2 -> O2 + 2 O} & \num{3.321e-9} & \num{-1.5} & \num{8.197e-19}\\
%\ch{O + O2 -> 3 O} & \num{1.660e-8} & \num{-1.5} & \num{8.197e-19}\\
% \end{tabular}
%\end{table}
The results for each temperature point were averaged over 100 samples.

%For exchange reactions we have Fig.~(\ref{fig:rate_const_NO_O}).
%\begin{figure}
%    \includegraphics[width=0.45\textwidth]{figures/NO_O_compare_FP_Arr_dt_1e-07_fnum_10000000.0_nrho1e+23.png}
%    \caption{\label{fig:rate_const_NO_O} Rate constant for $\ch{N2 + N}$ comparison calculated using the Arrhenius equation and reproduced from FP simulations.}
%\end{figure}
The evaluated results of the simulations can be seen in Fig.~(\ref{fig:rate_const_combined_dissocitaion}).
\begin{figure}
\centering
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/O2_O2_compare_FP_Arr_dt_1e-10_fnum_100000_nrho1e+23.png}
\caption{\ch{O2 + O2 -> O2 + 2 O}}
\label{fig:left}
\end{subfigure}\vspace{0.03\textwidth}
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/O2_O_compare_FP_Arr_dt_1e-10_fnum_100000_nrho1e+23.png}
\caption{\ch{O + O2 -> 3 O}}
\label{fig:right}
\end{subfigure}
\caption{Combined dissociation of \ch{O2}.}
\label{fig:rate_const_combined_dissocitaion}
\end{figure}
The rate constants calculated from the FP simulations match very well the ones predicted by the Arrhenius equation showing that the evaluation of the reaction probabilities is correctly implemented.

\subsection{Reaction Kinetics, $k = \mm{const}$}
To investigate whether the chemical kinetics are reproduced correctly, as well as if the lower moments are conserved as expected,  we consider a dissociation reaction of diatomic nitrogen 
\begin{equation}
\ch{N2 + N ->[\textit{k}] 3 N},
\end{equation}
where the reaction rate has the form of
\begin{equation}
    r = k [\ch{N2}] [\ch{N}].
\end{equation}
Assuming an isolated system with a constant volume, a temperature-independent rate constant, and the reaction being neither endo- nor exothermic, an analytic solution for the time dependent number density can be found 
\begin{equation}
    n_{\ch{N2}}(t) = \frac{n_{\ch{N2}}(t_0) Q}{2 n_{\ch{N2}}(t_0) - \big(n_{\ch{N2}}(t_0) - n_{\mm{tot}}(t_0) \big) \exp\big(Q\,k\,t\big)}
\end{equation}
where
\begin{equation}
    Q = \big(n_{\ch{N2}}(t_0) + n_{\mm{tot}}(t_0) \big)
\end{equation}
and
\begin{equation}
    n_{\mm{tot}}(t_0) = n_{\ch{N2}}(t_0) + n_{\ch{N}}(t_0).
\end{equation}
For the verification test case a rate constant of $k=\SI{e-15}{\per\second\meter\tothe{6}}$ was chosen.
The remaining simulation parameters are summarized in Tab.~\ref{tab:values_analytical_dissociation}.
\begin{table}[h!]
\caption{\label{tab:values_analytical_dissociation}Simulation Parameters Used for Analytical Dissociation Test Case}
\centering
 \begin{tabular}{ccccc} 
$\Delta t / \si{\second}$ & $V / \si{\meter\cubed}$ & $w$ & $n_{\ch{N}}(t_0) / \si{\per\meter\cubed}$ & $n_{\ch{N2}}(t_0) / \si{\per\meter\cubed}$\\
 \hline
    \num{e-10} & \num{e-12} & \num{e6} & \num{2e20} & \num{9.8e21}\\
 \end{tabular}
\end{table}

The simulation was performed 5 times, each time using a different seed for random numbers.
The results  displayed in Fig.~(\ref{fig:analytic_dissociation}) are averaged over these 5 simulations.
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/Analytic_dissociation_nrho_new.png}
    \caption{\label{fig:analytic_dissociation} Chemical kinetics for \ch{N2 + N} dissociation using a constant rate constant of $k=\SI{1e-15}{\per\second\meter\tothe{6}}$.}
\end{figure}
Very good agreement is observed between the analytic result and the averaged simulation results produced by our chemistry model.
Mass and momentum are exactly conserved. %as can be seen in Fig.~(\ref{fig:analytic_dissociation_mass_conserv})  and Fig.~(\ref{fig:analytic_dissociation_momentum_conserv}) respectively.
%\begin{figure}
%    \includegraphics[width=0.45\textwidth]{figures/Analytic_dissociation_mass.png}
%    \caption{\label{fig:analytic_dissociation_mass_conserv} Mass conservation.}
%\end{figure}
%\begin{figure}
%    \includegraphics[width=0.45\textwidth]{figures/Analytic_dissociation_momentum.png}
%    \caption{\label{fig:analytic_dissociation_momentum_conserv} Momentum conservation.}
%\end{figure}
The energy is conserved but the output is subject to noise as seen in Fig.~(\ref{fig:analytic_dissociation_energy_conserv}).
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/Analytic_dissociation_energy.png}
    \caption{\label{fig:analytic_dissociation_energy_conserv} Energy conservation.}
\end{figure}
The reason for the noise is,  that energy is a second order moment of the velocity distribution function, coupled with SPARTA's output format for floating point values being restricted to 7 decimal digits by default.

\subsection{Reaction Kinetics, $k = f(T)$}
\label{sec:reaction_kinetcs_k_T}
Even for a spatially homogenous gas, in the presence of vibrational relaxation and/or multiple reactions, it is no longer possible to obtain an analytical solution for the system of master equations describing the thermochemical relaxation of the gas mixture. Therefore, a numerical solution of a multi-temperature system of master equations~\cite{nagnibeda2009non} as well as simulation results produced by the SPARTA DSMC code with the Total Collision Energy model (TCE) are used as reference solutions against which the proposed Fokker-Planck chemistry algorithm is verified.
We use the extension of the DSMC algorithm  introduced by Zhang and Schwartzentruber \cite{zhang_inelastic_2013} to model energy relaxation for gas mixtures.

The relaxation of internal degrees of freedom in the FP model was modeled by the master equation ansatz for VHS gas mixtures \cite{hepp_kinetic_2022}.
Temperature dependent relaxation collision numbers $Z$ for both rotational and vibrational relaxation where used \cite{bird_molecular_1994}.
Collision numbers for the relaxation  between two species $\alpha$ and $\beta$ are the averages between the individual species collision numbers
\begin{equation}
	Z_{\alpha, \beta}(T) = \frac{Z_{\alpha}(T) + Z_{\beta}(T)}{2}.
\end{equation}

We investigate exchange and dissociation reaction sets individually to verify the functionality.
For all cases the simulation domain for the DSMC and FP simulations is a cube with a side length of \SI{e-5}{\meter} and periodic boundary conditions.
The starting temperature of each simulation is chosen to be $T = \SI{10000}{\kelvin}$ with a total number density of $n = \SI{e23}{\per\meter\cubed}$.
The mole fraction of each species is set to be equal to $x = \num{0,2}$.
A particle weight of $w = \num{e-6}$ and a time step of $\Delta t = \SI{e-8}{\second}$ are used.

\subsubsection{Exchange}
We consider the exchange reactions presented in table~\ref{tab:air_chemistry_exchange} of the appendix.
%It must be noted that the selection energy for the reaction $\ch{O2 + N -> NO + O}$ is not the same as $E_a = 0$ but rather $\Delta E = \SI{2.2129e-19}{\joule}$.

Very good agreement between all models can be observed for the  temporal development of the number densities of the participating species as can be seen in Fig.~\ref{fig:nrho_exchange_2_reactions}.
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/exchange_2_reactions/nrho_exchange_new.png}
    \caption{\label{fig:nrho_exchange_2_reactions} Number density using both exchange reactions.}
\end{figure}
In all figures, REF refers to the continuum, multi-temperature model.
While the temperature profile agrees very well between DSMC and FP, small deviations can be observed in relation to the multi-temperature model as seen in Fig.~\ref{fig:temp_exchange_2_reactions}.
These minor differences may be attributed to differences in the modelling of vibrational relaxation between DSMC and the continuum approaches.
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/exchange_2_reactions/temp_exchange_new.png}
    \caption{\label{fig:temp_exchange_2_reactions} Temperature using both exchange reactions.}
\end{figure}

\subsubsection{Dissociation}
For the dissociation test case \ch{O2} and \ch{N2} reactions are used from the appendix Tables~\ref{tab:air_chemistry_o2_diss} and \ref{tab:air_chemistry_n2_diss} respectively.
Good agreement can be observed between all models for \ch{O2} and \ch{O} kinetics (seen in Fig~\ref{fig:nrho_dissociation_10_reactions}).
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/dissociation_10_reactions/nrho_new.png}
    \caption{\label{fig:nrho_dissociation_10_reactions} Number density using 10 dissociation reactions.}
\end{figure}
The agreement is also very good between FP and the multi-temperature model as seen in Fig.~\ref{fig:nrho_dissociation_10_reactions_N2_N} and shows slightly larger deviations in respect to the DSMC results.
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/dissociation_10_reactions/nrho_N2_N.png}
    \caption{\label{fig:nrho_dissociation_10_reactions_N2_N} Number density of \ch{N2} and \ch{N} using 10 dissociation reactions (detail).}
\end{figure}
This shouldn't distract from the fact that the relative deviations are still small.
The same holds true for the temporal development of the translational temperature as displayed in Fig.~\ref{fig:temp_dissociation_10_reactions}.
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/dissociation_10_reactions/temp_new.png}
    \caption{\label{fig:temp_dissociation_10_reactions} Temperature using 10 dissociation reactions.}
\end{figure}
The slightly larger differences between the models in the temperature profile compared to results from exchange reactions are expected as now a considerably larger number of reactions is considered with a much larger temperature drop over the run of the simulation.
Due to this rapid evolution of the system, the differences in the modeling of vibrational relaxation between the considered approaches are exacerbated, leading to more noticeable differences in the temperature.
In addition, the use of the temperature-dependent collision numbers with the Larsen--Borgnakke model may lead to the model not satisfying detailed balance \cite{eckert_enforcing_2022}, an issue which is not present in the continuum-based approach, thus further affecting the evolution of the temperature.
However, this shouldn't distract from the fact that the relative deviations both in the number densities and the temperature are still small. 
